Meta Learning of Interface Conditions for Multi-Domain Physics-Informed Neural Networks

Physics-informed neural networks (PINNs) are emerging as popular mesh-free solvers for partial differential equations (PDEs). Recent extensions decompose the domain, apply different PINNs to solve the problem in each subdomain, and stitch the subdomains at the interface. Thereby, they can further alleviate the problem complexity, reduce the computational cost, and allow parallelization. However, the performance of multi-domain PINNs is sensitive to the choice of the interface conditions. While quite a few conditions have been proposed, there is no suggestion about how to select the conditions according to specific problems. To address this gap, we propose META Learning of Interface Conditions (METALIC), a simple, efficient yet powerful approach to dynamically determine appropriate interface conditions for solving a family of parametric PDEs. Specifically, we develop two contextual multi-arm bandit (MAB) models. The first one applies to the entire training course, and online updates a Gaussian process (GP) reward that given the PDE parameters and interface conditions predicts the performance. We prove a sub-linear regret bound for both UCB and Thompson sampling, which in theory guarantees the effectiveness of our MAB. The second one partitions the training into two stages, one is the stochastic phase and the other deterministic phase; we update a GP reward for each phase to enable different condition selections at the two stages to further bolster the flexibility and performance. We have shown the advantage of METALIC on four bench-mark PDE families.

==> exp2.tex <==
%\vspace{-0.1in}
\section{Experiment}

To evaluate \ours, we considered four benchmark equation families. We list the equations and domain decomposition settings in the following. 

\noindent \textbf{The Poisson Equation.} First, we considered a 2D Poisson equation with a parameterized source function, 
\begin{align}
	u_{xx} + u_{yy} = \widetilde{f}(x, y;s)
\end{align}
where $(x, y) \in [0, 1] \times [0, 1]$,  $\widetilde{f}(x, y;s) = f(x, y;s)/\max_{x,y} f(x, y; s)$, and
\begin{align}
	&f(x, y; s) = \left[\text{erf}( (x - 0.25)s) - \text{erf}((x- 0.75)s)\right] \notag \\
	&\cdot \left[\text{erf}((y - 0.25 )s) - \text{erf}((y-0.75)s)\right], 
\end{align}
where $\text{erf}(z)= \frac{2}{\sqrt{\pi}}\int_0^z e^{-t^2} \d t$, and $s \in [0, 50]$ is called the sharpness parameter that controls the sharpness of the interior square in the source. We used Dirichlet boundary conditions, and ran a finite difference solver to obtain an accurate ``gold-standard'' solution. To run multi-domain \pinns, we split the domain into two subdomains, where the interface is a line at $y = 0.5$. We visualize an exemplar solution and the subdomains, including the sampled boundary and collocation points in Fig. \ref{fig:poisson-vis}.   
\begin{figure}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/soln_Poisson.pdf}
			\caption{\small Solution at $s=20$}
		\end{subfigure} &
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/split_Poisson.pdf}
			\caption{\small Subdomains}
		\end{subfigure}
	\end{tabular}
	\caption{\small The Poisson equation. The interface is the green line at $y=0.5$. Blue and black dots show the sampled boundary points in each subdomain, and the internal dots (red and cyan) are the sampled collocation points inside each subdomain.} \label{fig:poisson-vis}
\end{figure}

%\subsection{Advection Equation}\label{sect:advec}
\noindent \textbf{Advection Equation.} We next considered a 1D advection (one-way wave) equation, $$ u_t + \beta u_x = 0$$ where $x \in [0, 2\pi]$, $t \in [0, 1]$, and $\beta$ is the PDE parameter denoting the wave speed.  We used Dirichlet boundary conditions, and the solution has an analytical form, $u(x, t) = h(x - \beta t)$ were $h(x)$ is the initial condition (which we select as $h(x)=\sin(x)$). For domain decomposition, we split the domain at $t= 0.5$ to obtain two subdomains. Fig. \ref{fig:advec-vis} shows an exemplar solution  and the subdomains with the interface. 
\begin{figure}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/soln_Advec.pdf}
			\caption{\small Solution at $\beta=30$ }
		\end{subfigure} &
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/split_Advec.pdf}
			\caption{\small Subdomains}
		\end{subfigure}
	\end{tabular}
	\caption{\small Advection equation. The interface is the green line at $t=0.5$.} \label{fig:advec-vis}
\end{figure}

%\subsection{Reaction Equation}\label{sect:react}
\noindent \textbf{Reaction Equation.} Third, we evaluate a 1D reaction equation, $$ u_t - \rho u(1-u) = 0 $$ where $\rho$ is the reaction coefficient (ODE parameter), $x \in [0, 2\pi]$, $t \in [0, 1]$ and $u(x, 0) = e^{-\frac{(x-\pi)^2}{2 (\pi/4)^2}}$. The exact solution is $u(x,t) = u(x, 0)\cdot[e^{\rho t}/\left(u(x,0)e^{\rho t} + 1 - u(x, 0)\right)]$. We split the domain at $t=0.5$ to obtain two subdomains. Although not required for well-posedness of the ODE system, because we are solving for the PINN space-time field $u(x,t)$, we use the exact solution to define a boundary loss term.  This enhances training without compromising the time partitioning we wish to highlight. We show a solution example and the subdomains in Fig. \ref{fig:reaction-vis}. 


%\subsection{Burger's Equation}\label{sect:burgers}
\noindent \textbf{Burger's Equation.} Fourth, we considered the viscous Burger's equation,  $$u_t + u u_x = \nu u_{xx}$$ where $\nu \in [0.001, 0.05]$ is the viscosity (PDE parameter), $x \in [-1, 1]$,  $t \in [0, 1]$, and $u(x, 0) = -\sin(\pi x)$. We ran a numerical solver to obtain an accurate ``gold-standard'' solution. To decompose the domain, we take the middle portion that  includes the shock waves as one subdomain, namely, $\Omega_1: x\in [-0.1, 0.1], t \in [0, 1]$, and the remaining as the other subdomain, $\Omega_2: x \in [-1, -0.1] \cap [0.1, 1], t \in [0, 1]$. Hence, the interface consists of two lines. See Fig. \ref{fig:burgers-vis} for the illustration and solution example. 

\begin{figure}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/soln_Reaction.pdf}
			\caption{\small Solution at $\rho=5.0$}
		\end{subfigure} &
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/split_Reaction.pdf}
			\caption{\small Subdomains}
		\end{subfigure}
	\end{tabular}
	\caption{\small Reaction equation. The interface is at $t=0.5$.} \label{fig:reaction-vis}
\end{figure}

\begin{figure}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/soln_Burgers.pdf}
			\caption{\small Solution at $\nu=0.001$ }
		\end{subfigure} &
		\begin{subfigure}[t]{0.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/split_Burgers.pdf}
			\caption{\small Subdomains}
		\end{subfigure}
	\end{tabular}
	\caption{\small Burger's equation. The interfaces are at $x=-0.1$ and $x=0.1$. The middle portion (filled with cyan dots) is the first subdomain, and the remaining parts constitute the  second subdomain.} \label{fig:burgers-vis}
% 	\vspace{-0.2in}
\end{figure}
\begin{figure*}
% 	\vspace{-0.1in}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Poisson_one_train.pdf}
			\caption{\small Poisson equation}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Advec_one_train.pdf}
			\caption{\small Advection equation}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Reaction_one_train.pdf}
			\caption{\small Reaction equation}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Burgers_one_train.pdf}
			\caption{\small Burgers' equation}
		\end{subfigure}
	\end{tabular}
%\vspace{-0.1in}
	\caption{\small Online performance of \ours-single. } \label{fig:accu-mab-single}
	%\vspace{-0.2in}
\end{figure*}	
\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}	
	\begin{tabular}[c]{cccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Poisson_two_train.pdf}
			\caption{\small Poisson equation}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Advec_two_train.pdf}
			\caption{\small Advection equation}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Reaction_two_train.pdf}
			\caption{\small Reaction equation}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs-xpinn-mab/errs/Burgers_two_train.pdf}
			\caption{\small Burgers' equation}
		\end{subfigure}
	\end{tabular}
%	\vspace{-0.05in}
	\caption{\small Online performance of \ours-seq.} \label{fig:accu-mab-seq}
%	\vspace{-0.1in}
\end{figure*}
\begin{figure}
	\vspace{-0.5in}
	\centering
	\setlength\tabcolsep{0pt}	
	\begin{tabular}[c]{c}
		\begin{subfigure}[b]{0.96\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Poisson.pdf}
			\caption{\small Poisson equation ($s=46.1$)}
			\label{fig:poisson}
		\end{subfigure}
		\\
		\begin{subfigure}[b]{0.96\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Advec.pdf}
			\caption{\small Advection equation ($\beta=24.02$)}
			\label{fig:advec}
		\end{subfigure}
		\\
		\begin{subfigure}[b]{0.96\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Reaction.pdf}
			\caption{\small Reaction equation ($\rho=4.1$)}
			\label{fig:reaction}
		\end{subfigure}
		\\
		\begin{subfigure}[b]{0.96\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Burgers.pdf}
			\caption{\small Burgers' equation ($\nu=0.0036$)}
			\label{fig:burgers}
		\end{subfigure}
	\end{tabular}
% 	\vspace{-0.1in}
	\caption{\small Point-wise solution error.}
	\label{fig:point-wise}
% 	\vspace{-0.5in}
\end{figure}



To evaluate \ours, we used 9 interface conditions, which are listed in the supplementary material. For the \pinn in each subdomain, we used two layers, with 20 neurons per layer and tanh activation function. We randomly sampled 1,000 collocation points and 100 boundary points for each PINN. To inject the interface conditions, we then randomly sampled 101 interface points for the Poisson, advection and reaction equations, and 802 interface points for Burger's equation. 
We set $\lambda_b=20$ and $\lambda_I = 5$, which follows the insight of~\citep{wang2021understanding,wang2022and} to adopt large weights for the boundary and interface terms so as to prevent the training of \pinns from being dominated by the residual term. 
We denote our single MAB by \ours-single, and sequential MABs by \ours-seq. For the latter, we set the discount factor $\gamma = 0.9$ (see \eqref{eq:reward-mab-1}). For better numerical stability, we used the relative $L_2$ error in the log domain to obtain the reward for updating the GP surrogate models. The running of the multi-domain \pinns consists of 10K ADAM epochs (with learning rate $10^{-3}$) and then 50K L-BFGS iterations (the first order optimality and parameter change tolerances set to $10^{-6}$ and $10^{-9}$ respectively). We set $c=1$ to compute the UCB score. We ran 200 plays (trials) for our method.  For static (offline) test, we randomly sampled 100 PDEs (which do not overlap with the PDEs sampled during the online playing). We then used the learned reward model to determine the best interface conditions for each particular PDE (according to the predictive mean), with which we ran the multi-domain \pinns to solve the PDE, and computed the relative $L_2$ error.  
\begin{table*}[t]
% 	\small
	\centering
    \resizebox{\columnwidth}{!}{%
	\begin{tabular}[c]{ccccc}
		\toprule
		{Method} & {Poisson} & Advection & Reaction & Burger's  \\
		\hline         
		Random-Single & 0.3992 $\pm$ 0.0037 & 0.07042 $\pm$ 0.01575 & 0.00612 $\pm$ 0.000278 & 0.04021 $\pm$ 0.00057\\
		Random-Seq &0.3004 $\pm$ 0.0032 & 0.03922 $\pm$ 0.00919& 0.01284$\pm$ 0.000707 & 0.03486 $\pm$ 0.00066 \\
		PINN-Sub & 0.03078 $\pm$ 0.00177 & 0.00130 $\pm$ 8.108e-5 & 0.00213 $\pm$ 0.00021 & 0.00738 $\pm$ 0.00313 \\
		PINN-Merge-H & 0.02398 $\pm$ 0.00144 & 0.00098 $\pm$ 5.038e-5 & 0.00223 $\pm$ 0.00026 & 0.00951 $\pm$ 0.00390 \\
		PINN-Merge-V & 0.02184 $\pm$ 0.00211 & 0.00079 $\pm$ 3.391e-5 & \textbf{0.00099} $\pm$ \textbf{0.00013} & 0.00276 $\pm$ 0.00041 \\
		\ours-Single-TS &0.02503 $\pm$ 0.0002 & 0.00079 $\pm$ 4.5897e-5 & 0.00204 $\pm$ 1.013e-4 & \textbf{0.00109} $\pm$ \textbf{1.306e-5} \\
		\ours-Single-UCB &0.0245$\pm$ 0.0002 & 0.00078 $\pm$ 3.6771e-5& 0.00102 $\pm$ 8.945e-6 & 0.00161 $\pm$ 2.939e-5 \\
		\ours-Seq-TS &0.01639$\pm$ 9.5384e-5 & 0.00078 $\pm$ 3.6473e-5 & \textbf{0.00099} $\pm$ \textbf{8.4704e-6} & 0.00152 $\pm$ 5.571e-5 \\
		\ours-Seq-UCB & \textbf{0.01406} $\pm$ \textbf{9.1099e-5} & \textbf{0.00070} $\pm$ \textbf{3.2790e-5} & \textbf{0.00099} $\pm$ \textbf{5.999e-6} & 0.00139 $\pm$ 3.948e-5 \\
		\bottomrule
	\end{tabular}
	}
	\caption{\small The average  $L_2$ relative error of single-domain \pinns and multi-domain \pinns for solving 100 test PDEs. The interface conditions of the multi-domain \pinns are provided by \ours and random selection. \{Single, Seq\} indicate using a single set or two sequential sets of interface conditions for the running of the multi-domain \pinns.  \{TS, UCB\} corresponds to our method using TS or UCB score to determine the interface conditions at each play.} \label{tb:test-result}
% 	\vspace{-0.1in}}}
\end{table*}

First, to examine the online performance of \ours, we looked into the accumulated solution error along with the number of plays. We compared with randomly selecting the arm at each play.  In the case of running \ours-seq, this baseline correspondingly randomly selects the arm twice, one at the stochastic training phase, and the other at the deterministic phase. The results are shown in Fig. \ref{fig:accu-mab-single} and \ref{fig:accu-mab-seq}. As we can see, the accumulated error of \ours with both UCB and TS grows much slower, \ie sublinearly, than the random selection approach (note that the reward of the optimal action is unknown due to the randomness in the running of PINNs, and we cannot compute the regret). This has shown  that our method achieves a much better exploration-exploitation tradeoff in the online interface condition decision and model updating, which is consist with many other MAB applications (see Sec \ref{sect:rel}). The results demonstrate the advantage of our MAB-based approach. First, via effective exploration, \ours can collect valuable training examples (rewards at new actions and context) to improve the learning efficiency and performance of the GP reward surrogate model. Second, the online decision also takes advantage of the predictive abaility of the current reward model, \ie exploitation, to select effective interface conditions, which results in increasingly better solution accuracy of the multi-domain \pinns. The online nature of \ours enables us to keep improving the reward model while utilizing it to solve new equations with promising accuracy. 

Next, we conducted an offline test, namely, without online exploration and model updates any more after 200 plays. We compared with (1) Random-Single, which, for each PDE, randomly selects a set of interface conditions applied to the entire training of the multi-domain PINNs, and (2) Random-Seq, which for each PDE, randomly selects two sets of interface conditions, one for the stochastic training and the other for the deterministic training phase. We also tested single-domain \pinns that do not incorporate interface conditions. Specifically, we compared with (3) \pinn-Sub, which used the same architecture as the PINN in each subdomain, but applied to the entire domain, (4) \pinn-Merge-H, which horizontally pieced all the \pinns in the subdomains, \ie doubling the layer width yet fixing the depth, (5) \pinn-Merge-V, which vertically stacked the \pinns, \ie doubling the depth while fixing the width.  Note that while \pinn-Merge-H and \pinn-Merge-V merge the \pinns in each subdomain, the total number of neurons actually increases (for connecting these \pinns). Hence, the merged \pinn is more expressive. 
Each single-domain \pinn used the union of the boundary points and collocation points from every subdomain. We used the same weight for the boundary term, \ie $\lambda_b= 20$. The running of each single-domain \pinn follows exactly the same setting of the multi-domain \pinns (\ie 10K ADAM epochs and 50K L-BFGS iterations). 

We report the average relative $L_2$ solution error and the standard deviation in Table \ref{tb:test-result}. As we can see, randomly selecting interface conditions, no matter for the whole training procedure or two training phases, result in much worse solution accuracy of multi-domain \pinns. The solution error is one order of magnitude  bigger than \ours in all the settings. It confirms that the success of the multi-domain \pinns is up to appropriate interface conditions. Next, we can observe that while the performance of \ours-Single is similar to \ours-Seq, the best solution accuracy is in most cases obtained by interface conditions selected by \ours-Seq (except in solving the Burger's equation). It demonstrates that our sequential MAB model that can employ different conditions for the two training phases is more flexible and brings additional improvement. We also observe that in most cases using the UCB for online playing can lead to better performance for both \ours-Single and \ours-Seq. This is consistent with the online performance evaluation (see Fig. \ref{fig:accu-mab-single} and \ref{fig:accu-mab-seq}). Third, among the single-domain PINN methods, PINN-Merge-V outperforms PINN-sub in all the equation families and PINN-Merge-H outperforms PINN-sub in the Poisson and advection equations, showing that deeper or wider architectures can help further improve the solution accuracy. However, their performance is still second to the best setting of \ours, which uses simpler  subdomain PINN  architectures and fewer total learnable parameters. These multi-domain PINNs can be further  parallelized to accelerate training. By contrast, if the interface conditions are inferior, such as those selected by Random-Single and Random-Seq, the solution error becomes much worse (orders of magnitude bigger) than single-domain PINNs. Together these results  have shown the importance of the interface conditions for multi-domain \pinns and the advantage of our method. 

For a fine-grained comparison, we visualize the point-wise solution error  of \pinn-Sub, Random-Single, Random-Seq, and our method in solving four random instances of the equations. As shown in Fig. \ref{fig:point-wise}, the point-wise error of both \ours-Single and \ours-Seq  is quite uniform across the domain and close to zero (dark blue). By contrast, the competing methods often exhibit relative large errors in a few local regions, \eg those in the middle (where the shock waves appear) of the domain of the Burger's equation (PINN-Sub, Random-Single, Random-Seq), and the central part of the domain of the Poisson and advection equation (Random-Single). It shows that our method not only can give a superior global accuracy, but locally also better recovers individual solution values.

Finally, we analyzed the selected interface conditions in each equation family by \ours. We found that those conditions are interesting,  physically meaningful, and consistent with the properties of the equations. Due to the space limit, we provide the detailed analysis and discussion in the supplementary material. 


\cmt{
	\begin{figure}[!htb]
		\centering
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Poisson_query.pdf}
			\caption{\small Poisson $s=46.1$}
			\label{fig:poisson}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Advec_query.pdf}
			\caption{\small Advec $\beta=24.02$}
			\label{fig:advec}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Reaction_query.pdf}
			\caption{\small Reaction $\rho=4.1$}
			\label{fig:reaction}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Burgers_query.pdf}
			\caption{\small Burgers $\nu=0.0036$}
			\label{fig:burgers}
		\end{subfigure}
		%\vspace{-0.1in}
		\caption{\small \ours-Single, Ground solutions and errors field}
		\label{fig:pred-top-structure}
		%\vspace{-0.2in}
	\end{figure}
}
\cmt{
	\begin{figure}[!htb]
		\centering
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Poisson_step2.pdf}
			\caption{\small Poisson $s=46.1$}
			\label{fig:poisson}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Advec_step2.pdf}
			\caption{\small Advec $\beta=24.02$}
			\label{fig:advec}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Reaction_step2.pdf}
			\caption{\small Reaction $\rho=8.2$}
			\label{fig:reaction}
		\end{subfigure}
		\begin{subfigure}[b]{0.43\textwidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figs-xpinn-mab/preds/preds_Burgers_step2.pdf}
			\caption{\small Burgers $\nu=0.0036$}
			\label{fig:burgers}
		\end{subfigure}
		%\vspace{-0.1in}
		\caption{\small \ours-Seq, Ground solutions and errors field}
		\label{fig:pred-top-structure}
		%\vspace{-0.2in}
	\end{figure}
}



